Experimental Design in Two-Sided Platforms: An Analysis of Bias

We develop an analytical framework to study experimental design in two-sided marketplaces. Many of these experiments exhibit interference, where an intervention applied to one market participant influences the behavior of another participant. This interference leads to biased estimates of the treatment effect of the intervention. We develop a stochastic market model and associated mean field limit to capture dynamics in such experiments, and use our model to investigate how the performance of different designs and estimators is affected by marketplace interference effects. Platforms typically use two common experimental designs: demand-side ("customer") randomization (CR) and supply-side ("listing") randomization (LR), along with their associated estimators. We show that good experimental design depends on market balance: in highly demand-constrained markets, CR is unbiased, while LR is biased; conversely, in highly supply-constrained markets, LR is unbiased, while CR is biased. We also introduce and study a novel experimental design based on two-sided randomization (TSR) where both customers and listings are randomized to treatment and control. We show that appropriate choices of TSR designs can be unbiased in both extremes of market balance, while yielding relatively low bias in intermediate regimes of market balance.

==> TSR_old.tex <==
\subsection{Estimation with the $\TSR$ design}
%\label{ssec:TSR_est}

The preceding section reveals that each of the naive $\LR$ and $\CR$ estimators has its virtue, depending on market balance conditions.  In this section, we explore whether we can develop $\TSR$ designs and estimators in which $a_C$ and $a_L$ are chosen {\em as a function of} $\lambda/\tau$, to obtain the beneficial asymptotic performance of the naive $\CR$ estimator in the highly-demand constrained regime, as well as the $\LR$ estimator in the highly supply-constrained regime. \newgw{We also explore the performance of $\TSR$ in intermediate regimes of market balance.}

Recall the naive $\TSR$ estimator defined in \eqref{eq:naive_TSR_est}, and in particular the steady-state version of this estimator.  Suppose the \newgw{platform} \delgw{market} observes $\lambda/\tau$; note that this is reasonable from a practical standpoint as this is a measure of market imbalance involving only the overall arrival rate of customers and the average rate at which listings become available.  For example, consider the following heuristic choices of $a_C$ and $a_L$ for the $\TSR$ design, for some fixed values of $\b{a}_C$ and $\b{a}_L$:
\begin{equation}
a_C(\lambda/\tau) = \left(1 - e^{-\lambda/\tau}\right) + \b{a}_C e^{-\lambda/\tau}; \quad a_L(\lambda/\tau) = \b{a}_L\left(1 - e^{-\lambda/\tau}\right) + e^{-\lambda/\tau}. \label{eq:aC_aL_naive_TSR}
\end{equation}
Then as $\lambda/\tau \to 0$, we have $a_C(\lambda/\tau) \to \b{a}_C$ and $a_L(\lambda/\tau) \to 1$, while as $\lambda/\tau \to \infty$ we have $a_C(\lambda/\tau) \to 1$ and $a_L(\lambda/\tau) \to \b{a}_L$.\footnote{Our choice of exponent here is somewhat arbitrary; the same analysis follows even if we replace $e^{-\lambda/\tau}$ with $e^{-c\lambda/\tau}$ for any value of $c > 0$.}. With these choices, it follows that in the highly demand-constrained limit ($\lambda/\tau \to 0$), the naive $\TSR$ estimator becomes equivalent to the naive $\CR$ estimator, while in the highly supply-constrained limit ($\lambda/\tau \to \infty$), the naive $\TSR$ estimator becomes equivalent to the naive $\LR$ estimator.  In particular, using Propositions \ref{prop:Qij_demand_constrained} and \ref{prop:Qij_supp_constrained}, it is straightforward to show that the steady-state naive $\TSR$ estimator is unbiased in {\em both} limits; we state this as the following theorem, and omit the proof.%\footnote{The result only requires the fact that $1 - e^{-x}/x \to 0$ as $x \to 0$.}
%\gw{Should this be a corollary instead of a theorem?}
\begin{corollary}
\label{cor:naive_TSR}
For each $\lambda/\tau$, consider the $\TSR$ design with $a_C$ and $a_L$ defined as in \eqref{eq:aC_aL_naive_TSR}.  Consider a sequence of systems where either $\lambda/\tau \to 0$, or $\lambda/\tau \to \infty$.  Then in either limit:
\[ \widehat{\GTE}^{\TSR}(\infty | a_C(\lambda/\tau), a_L(\lambda/\tau)) - \GTE\to 0. \]
\end{corollary}

Figure \ref{fig:numerics} reveals the steady-state performance of the different naive estimators ($\CR$, $\LR$, and $\TSR$ with the preceding scaling of $a_C$ and $a_L$), as a function of market balance $\lambda/\tau$.  The figure shows the difference between each estimator and $\GTE$; the estimators are all upward-biased because of the parameter values chosen, though the qualitative findings in the figure are robust across parameter choices.  As we see, the naive $\TSR$ estimator performs well in each asymptotic regime.

We are also led to ask whether we can improve upon the naive $\TSR$ estimator when the market is moderately balanced.  %Note that the naive $\TSR$ estimator interpolates in between $\LR$ and $\CR$ changing the weights as a function of market balance to take advantage of the virtues of each estimator. However, 
Note that the naive $\TSR$ estimator does not explicitly correct for {\em either} the fact that there is interference across listings, or the fact that there is interference across customers. We now suggest a heuristic for correction of these effects that leads to an improved interpolating $\TSR$ estimator; this is the fourth estimator that appears in Figure \ref{fig:numerics}, \newgw{that we call `Improved $\TSR$'}.  

First, abusing notation, let $\GTE^{\CR}(T|a_C, a_L)$ denote the estimator in \eqref{eq:naive_CR} using the same terms from a $\TSR$ design, and  dividing through by $a_L$ on both terms as normalization.  Similarly abusing notation,  let $\GTE^{\LR}(T|a_C, a_L)$ denote the estimator in \eqref{eq:naive_CR} using the same terms from a $\TSR$ design, and dividing through by $a_C$ on both terms as normalization.  Motivated by these naive estimators, we explicitly consider an interpolation between the $\LR$ and $\CR$ estimators of the form:
\newgw{\begin{align}
\label{eq:interpolatingTSR}
 \beta \widehat{\GTE}^{\CR}(T|a_C,a_L)+(1-\beta)\widehat{\GTE}^{\LR}(T|a_C,a_L)& \\ = \beta \left(\frac{Q_{11}(T | a_C,a_L)}{a_Ca_L} - \frac{Q_{01}(T | a_C,a_L)}{(1-a_C)a_L}\right) &+ (1-\beta) \left(\frac{Q_{11}(T | a_C,a_L)}{a_Ca_L} - \frac{Q_{10}(T | a_C,a_L)}{a_C(1-a_L)}\right). \notag
 \end{align}}
 

Now, consider the quantity $Q_{00}(T|a_C,a_L)/((1-a_C)(1-a_L)) - Q_{10}(T|a_C,a_L)/((1-a_C)a_L)$ in a $\TSR$ design. This is the (appropriately normalized) difference between the rate at which control customers book control listings, and the rate at which treatment customers book control listings.   Note that the  difference between control customers and treatment customers is that the latter are exposed to treatment listings, while the former are not. Hence, the difference in steady-state rates of booking among these two groups on {\em control listings} must be driven by the fact that treatment customers substitute booking from control listings to treatment listings (or vice versa). This difference is precisely the ``cannibalization" effect (i.e., interference) that was found in $\LR$ designs in the highly demand-constrained regime.

Following from this motivation, we subtract an appropriately weighted ``correction term’’ for the $\LR$ design from our interpolating $\TSR$ estimator in \eqref{eq:interpolatingTSR}. 
(This argument is of course heuristic: it ignores dynamic effects in regimes of intermediate market balance.) %\gw{Not sure what to say about scaling bias. Probably nothing at this point}.
Using a symmetric argument we also subtract an appropriately weighted correction term associated to interference across customers in a $\CR$ design:  $Q_{00}(T|a_C,a_L)/((1-a_L)(1-a_C))-Q_{01}(T|a_C,a_L)/((1-a_C)a_L)$.  (Similar correction terms were also studied in \cite{bajari2019double}; see the related work for further details on this work.)
We weight these 
correction terms in a market-balance-dependent fashion, based on the direction of market balance in which we have seen that the respective interference grows.  Combining these insights, for $\beta \in (0,1)$ our improved $\TSR$ estimator is given by:
\begin{multline}
\label{eq:TSRI}
\widehat{\GTE}^{\TSRI}(T|a_C, a_L) = \\
\beta \left[\frac{Q_{11}(T | a_C,a_L)}{a_Ca_L} - \frac{Q_{01}(T | a_C,a_L)}{(1-a_C)a_L}-(1-\beta)\left(\frac{Q_{00}(T|a_C, a_L)}{(1-a_C)(1-a_L)}-\frac{Q_{01}(T|a_C, a_L)}{(1-a_C)a_L}\right) \right] \\
+(1- \beta) \left[ \frac{Q_{11}(T | a_C,a_L)}{a_Ca_L} - \frac{Q_{10}(T | a_C,a_L)}{a_C(1-a_L)}-\beta\left(\frac{Q_{00}(T|a_C,a_L)}{(1-a_C)(1-a_L)}-\frac{Q_{10}(T|a_C,a_L)}{a_C(1-a_L)}\right) \right],
\end{multline}
Given market balance $\lambda/\tau$, we set $\beta=e^{-\lambda/\tau}$, and we choose $a_C$ and $a_L$ as in \eqref{eq:aC_aL_naive_TSR}.

In the limit where $\lambda/\tau \to 0$, note that $\widehat{\GTE}^{\TSRI} (T|a_C(\lambda/\tau),a_L(\lambda/\tau))\to\widehat{\GTE}^{\CR}(T|\b{a}_C)$ as expected.  Similarly, in the limit where $\lambda/\tau \to \infty$, we have $\widehat{\GTE}^{\TSRI} (T|a_C(\lambda/\tau),a_L(\lambda/\tau))\to\widehat{\GTE}^{\LR}(T|\b{a}_L)$.  In particular, it is straightforward to show as a result that this new estimator is also unbiased in {\em both} the highly demand-constrained and highly supply-constrained regimes.  In these limits, the correction terms play no role.  However, for moderate values of market balance,  both the cannibalization correction terms kick in, \newgw{improving over naive $\TSR$ as seen in the figure. As we mentioned, we leave the study of other $\TSR$ designs and estimators that may perform even better for future research.}

\gw{Figure 1: should we normalize by GTE as in the next figure?  Can we provide an appendix with more results to give more sense of robustness?}


\begin{figure}
    \centering
    \begin{tabular}{c c}
     \includegraphics[width=0.5\textwidth]{estimator_minus_gte_lambdas.pdf}
    &  
    \includegraphics[width=0.5\textwidth]{transient_dynamics_med_lambda.pdf}
    \end{tabular}
    \caption{Left: Difference between estimator and $\GTE$ in steady state.  We consider variation in $\lambda/\tau$ by fixing $\tau = 1$ and varying $\lambda$; analogous results are obtained if $\lambda$ is fixed and $\tau$ is varied.  Right: transient behavior of estimators. Again we fix $\tau = 1$.  For both plots, we set $\epsilon_{\gamma,i}=1, \alpha_{\gamma,i}=0.5$ for all $\gamma, i$. In the $\CR$ design, $a_C=1/2$. In the $\LR$ design, $a_L=1/2$. There are three listing types and two customer types.
    %: $\{\theta_1, \theta_2, \theta_3\}$. Customer types:$\{\gamma_1, \gamma_2\}$.
    Utilities for $\gamma_1$ are $v_{\gamma_1}(\theta_1)= 1.5, v_{\gamma_1}(\theta_2)=3 , v_{\gamma_1}(\theta_3)=6.
    \tilde{v}_{\gamma_1}(\theta_1)= 1,
    \tilde{v}_{\gamma_1}(\theta_2)=8,
    \tilde{v}_{\gamma_1}(\theta_3)=12.$
    Utilities for $\gamma_2$ are $v_{\gamma_2}(\theta_1= 1, v_{\gamma_2}(\theta_2)=2 , v_{\gamma_2}(\theta_3)=4.
    \tilde{v}_{\gamma_2}(\theta_1)= 0.5,
    \tilde{v}_{\gamma_2}(\theta_2)=6,
    \tilde{v}_{\gamma_2}(\theta_3)=8$.}
    \label{fig:numerics}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=.5]{estimator_minus_gte_taus.pdf}
%     \caption{Caption}
%     \label{fig:est_minus_gte_taus}
% \end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> transient.tex <==

\subsection{Transient behavior}

For practical implementation, it is important to consider the relative bias in the candidate estimators in the transient system, since experiments are typically run for relatively short time horizons. 
Theoretically, we can provide some insight when $\tau \to \infty$: in this case, the dominant term in the right hand side of \eqref{eq:ODE} is $(\rho(\theta) - s_t(\theta))\tau$.  Using this fact, it can be shown that as $\tau \to \infty$, for each $t > 0$, there holds $\v{s}_t^*(a_C, a_L) \to \v{\rho}(a_L)$ (where we define $\v{\rho}(a_L)$ as in Section \ref{ssec:ss_theory}).  In other words, the state {\em remains} at $\v{\rho}(a_L)$ at all times.   As a result in this limit the transient estimators $\widehat{\GTE}^{\CR}(T | a_C)$ and $\widehat{\GTE}^{\LR}(T | a_L)$ are equivalent to $\widehat{\GTE}^{\CR}(\infty | a_C)$ and $\widehat{\GTE}^{\LR}(\infty | a_L)$, respectively.  In particular, asymptotically as $\tau \to \infty$, the transient estimator $\widehat{\GTE}^{\CR}(T | a_C, a_L)$ will be an {\em unbiased} estimate of $\GTE$ at all times $T > 0$.  (The same is true if $\lambda \to 0$, provided the initial state is $\v{s}_0 = \v{\rho}(a_L)$.)

More generally, Figure \ref{fig:transient_dynamics} numerically investigates how the time horizon of the experiment affects the performance of the estimators in the mean field model; there we plot an example where $\lambda/\tau$ takes a moderate value.  The relative performance of estimators depends on the time horizon of interest as well as market balance conditions. 

\begin{figure}[H]
    \centering
    \begin{tabular}{c c c }
        \includegraphics[height=0.26\textwidth]{figs_transient/dynamics_lam_01_mod.png}
        &
        \includegraphics[height=0.26\textwidth]{figs_transient/dynamics_lam_1_mod.png}
        & 
        \includegraphics[height=0.26\textwidth]{figs_transient/dynamics_lam_10_mod.png}
    \end{tabular}
    \caption{Transient dynamics of estimators with $\lambda/\tau = 0.1, 1$, and $10$. Parameters are as defined in Figure \ref{fig:numerics}.}
    \label{fig:transient_dynamics}
\end{figure}






